Unified Interpretation of Softmax Cross-Entropy and Negative Sampling: With Case Study for Knowledge Graph Embedding

In knowledge graph embedding, the theoretical relationship between the softmax cross-entropy and negative sampling loss functions has not been investigated. This makes it difficult to fairly compare the results of the two different loss functions. We attempted to solve this problem by using the Bregman divergence to provide a unified interpretation of the softmax cross-entropy and negative sampling loss functions. Under this interpretation, we can derive theoretical findings for fair comparison. Experimental results on the FB15k-237 and WN18RR datasets show that the theoretical findings are valid in practical settings.

==> header.tex <==
 \usepackage[nonatbib,final]{neurips_2020}

\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography

%%%%%%%%%%%%%%

%% And abstract
\usepackage{times}
\usepackage{latexsym}
%\renewcommand{\UrlFont}{\ttfamily\small}

%\usepackage[hyperref]

%\newcommand{\mat}[1]{\boldsymbol{\mathbf{#1}}}
\newcommand{\mat}[1]{\mathbf{\boldsymbol{#1}}}
%\usepackage{mathtools}
\newcommand{\transposeb}{^{(b)\mathrm{T}}}

\newcommand{\argmax}{\mathop{\rm argmax}\limits}
\newcommand{\argmin}{\mathop{\rm argmin}\limits}
\newcommand{\Cset}{\mathbb{C}}
\newcommand{\Rset}{\mathbb{R}}

\newcommand{\Y}{\mathcal{Y}}

\usepackage{pifont}
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%

\newcommand{\fixme}[1]{{\small\color{blue!40!green}[FIX ME: #1]}}

\usepackage{soul}
\usepackage{url}
\usepackage[utf8]{inputenc}
\usepackage[small]{caption}

%\usepackage[dvipdfmx]{graphicx}
\usepackage[dvipdfmx]{xcolor}

\definecolor{mycolor}{RGB}{255,51,76}

\usepackage{tabu}
\usepackage{tabularx}
\usepackage{multirow}
\usepackage{array}
\usepackage{amsfonts}
\usepackage{bm}

\usepackage{booktabs}
\usepackage{mathptmx}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsthm}
\newtheorem{prop}{Proposition}
\usepackage{algorithm,algorithmic}
\renewcommand{\algorithmiccomment}[1]{{\scriptsize\sl // #1}}

\usepackage[above,below]{placeins}

%\usepackage[upright]{fourier}
\DeclareMathAlphabet{\mathcal}{OMS}{zplm}{m}{n}
\usepackage{mathtools}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "ijcai20"
%%% End:

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "ijcai20"
%%% End:

\usepackage{natbib}
